agriFrame: Agricultural framework to remotely control a rover inside a greenhouse environment

The growing demand for innovation in agriculture is essential for food security worldwide and more implicit in developing countries. With growing demand comes a reduction in rapid development time. Data collection and analysis are essential in agriculture. However, considering a given crop, its cycle comes once a year, and researchers must wait a few months before collecting more data for the given crop. To overcome this hurdle, researchers are venturing into digital twins for agriculture. Toward this effort, we present an agricultural framework(agriFrame). Here, we introduce a simulated greenhouse environment for testing and controlling a robot and remotely controlling/implementing the algorithms in the real-world greenhouse setup. This work showcases the importance/interdependence of network setup, remotely controllable rover, and messaging protocol. The sophisticated yet simple-to-use agriFrame has been optimized for the simulator on minimal laptop/desktop specifications.

==> draft_content.tex <==
The use of robotics in agriculture can offer a promising solution to increase efficiency and sustainability. Mobile robots can help farmers to automate repetitive tasks, optimize crop growing conditions, and reduce resource waste by providing accurate and timely information about the status of crops, soil, and micro-climate. This can lead to better decision-making, higher yields, and lower costs. One potential application of robotics in agriculture is the development of autonomous greenhouse systems. These systems can monitor and control multiple environmental variables, such as temperature, humidity, light, and CO2, to create optimal growing conditions for crops. Autonomous greenhouse systems can also use machine learning algorithms to predict the impact of changes in environmental variables on crop growth and adjust the conditions accordingly. This can lead to significant improvements in crop yield and quality and a reduction in resource use and waste.

 
The deployment of robotics in agriculture offers a promising solution to enhance efficiency, sustainability, and food security. By automating repetitive tasks, optimizing crop growing conditions, and providing accurate and timely information, robots can help farmers to improve yields, reduce costs, and minimize the environmental impact of agriculture. As the demand for food continues to grow, developing and adopting robotic systems in agriculture will become increasingly important to ensure a sustainable and prosperous future for all.
\textcolor{red}{think of adding a figure in the intro itself, a very abstract figure}
The researchers \cite{ma2019greenhouse} addressed the issue of microclimates affecting greenhouse plant science assays, which introduced significant noise to plant growth measurement data. While randomizing pot locations helped redistribute the noise, it did not eliminate it entirely. The researchers proposed an approach to optimize the shuffling patterns of plants to eliminate the impacts of microclimates. To achieve this, they developed a computer modeling approach to simulate the microclimate within the greenhouse. The simulation model considered real design, materials, and location information from a specific greenhouse (Purdue Lily greenhouse in West Lafayette, Indiana). The researchers optimized the pot movement frequency and distance using the simulation results. By implementing a new shuffling pattern based on the simulation model, they were able to remove over 90\% of the microclimate variance. Furthermore, this optimized pattern required more than 95\% less shuffling effort than non-stop movement, thus providing a more efficient solution.

The major contributions of this paper are as follows:
\begin{itemize}
    \item Agricultural framework for deploying/teaching greenhouse rover as shown in Fig.~\ref{agri:frameowrk}.
    \item A framework to develop, simulate, and test on the remote hardware (Rover).
    \item Greenhouse simulator environment for a testing rover before deploying in the real world
    \item Networking for remotely controlling the rover with appropriate benchmarks.
\end{itemize}

\cite{choab2019review} have done a comprehensive literature review on greenhouse systems, focusing on identifying the preferable characteristics of greenhouses for different climates and operating conditions. The authors also address the selection process for greenhouse shape and orientation in different climates.

The simulation tool proposed in \cite{BAGLIVO2020115698} incorporates various factors that influence the thermal environment within a greenhouse, including external weather conditions, solar radiation, greenhouse design parameters, and crop characteristics. By considering these factors, the tool can simulate the dynamic behavior of the greenhouse and predict the temperature, humidity, and energy demand for different crop species. The tool's accuracy is validated through comparisons with real-world data, demonstrating its reliability and usefulness in practical applications.
